Network-Level Adversaries in Federated Learning

Federated learning is a popular strategy for training models on distributed, sensitive data, while preserving data privacy. Prior work identified a range of security threats on federated learning protocols that poison the data or the model. However, federated learning is a networked system where the communication between clients and server plays a critical role for the learning task performance. We highlight how communication introduces another vulnerability surface in federated learning and study the impact of network-level adversaries on training federated learning models. We show that attackers dropping the network traffic from carefully selected clients can significantly decrease model accuracy on a target population. Moreover, we show that a coordinated poisoning campaign from a few clients can amplify the dropping attacks. Finally, we develop a server-side defense which mitigates the impact of our attacks by identifying and up-sampling clients likely to positively contribute towards target accuracy. We comprehensively evaluate our attacks and defenses on three datasets, assuming encrypted communication channels and attackers with partial visibility of the network.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}


Our results shed light on the potential vulnerabilities of federated learning algorithms to network-level adversaries. 
Below we discuss how assumptions we made impact our results.


Our results hold for adversaries who target the accuracy of a subpopulation in the data, which only has data in a small number of clients. For next word prediction, this could be clients who use new slang or a geographically-relevant term, or clients who have observed a novel type of malware for a malware classification task. Our results would likely be unable to harm overall model performance, as a large fraction of clients would need to be removed to achieve this. In order to run our attacks, the target clients should be observable by the network adversary---if clients with similar behavior are close to each other geographically, a network adversary with more limited access can still harm the model significantly.

Our results show that more limited adversary access can seriously limit their effect. The adversary is much less effective when observing $\AggMean$ aggregation in \CTwo and \CThree than when observing $\AggEach$ aggregation in \COne; to prevent very powerful attacks, encrypted communication should certainly be used. Larger batch sizes $m$ may also lead to increased difficulty identifying specific target clients. Furthermore, an adversary who can also add poisoned clients can amplify attack performance significantly. Servers can and should use standard poisoning defenses such as update clipping to prevent the most powerful attacks.

Our defense strategy demonstrates that it is possible to identify helpful users when given access to a validation dataset of samples from a sensitive subpopulation. While our server had knowledge of the attack subpopulation when running upsampling, it is possible to collect data from several sensitive subpopulations to identify poor performing subpopulations and improve their performance. Our defense highlights the value of trusted information in Byzantine machine learning settings, including trusted validation sets or trusted participants. It is important to use these when available, but not overfit to them (otherwise, we could simply train on the trusted data rather than run the protocol)---our attacks have large impact on accuracy, so identifying and correcting the model does not rely heavily on the specific validation set. 
One interesting aspect of our work is that our dropping attack and upsampling defense use the same basic procedure, which is connected to well known problems in probability. While improvements are certainly possible for the defense, those same improvements should also be possible for the attack; it may be more fruitful to improve the gap in knowledge between the adversary and server, such as by using communication strategy \CTwo or identifying and communicating with trusted clients.

Our work did not consider the cost on the attacker in conducting these attacks on a real network, so they are an upper bound on the decrease in accuracy that can be created by selecting clients with significant contributions to the model. In practice, an attacker would require significant cost to conduct dropping attacks at clients that are geographically distributed vs, say clients that are all collocated in the same small, geographical location.  Our defense also can benefit from integrating geographical distribution in the set of clients to sample from. Selecting clients that are geographically distributed and thus have a higher attacker cost with respect to network-level attacks can significantly mitigate dropping attacks.


